SLOPE: Search with Learned Optimal Pruning-based Expansion

Heuristic search is often used for motion planning and pathfinding problems, for finding the shortest path in a graph while also promising completeness and optimal efficiency. The drawback is it's space complexity, specifically storing all expanded child nodes in memory and sorting large lists of active nodes, which can be a problem in real-time scenarios with limited on-board computation. To combat this, we present the Search with Learned Optimal Pruning-based Expansion (SLOPE), which, learns the distance of a node from a possible optimal path, unlike other approaches that learn a cost-to-go value. The unfavored nodes are then pruned according to the said distance, which in turn reduces the size of the open list. This ensures that the search explores only the region close to optimal paths while lowering memory and computational costs. Unlike traditional learning methods, our approach is orthogonal to estimating cost-to-go heuristics, offering a complementary strategy for improving search efficiency. We demonstrate the effectiveness of our approach evaluating it as a standalone search method and in conjunction with learned heuristic functions, achieving comparable-or-better node expansion metrics, while lowering the number of child nodes in the open list. Our code is available at https://github.com/dbokan1/SLOPE.

==> figures/table.tex <==
\begin{table*}[!htpb]
\small
\centering
\caption{Average expansions over test set (task loss) of different algorithms on different databases}
\begin{tabulary}{1.0\textwidth}{LCL|*{4}{C}} \toprule
 & {\bf World Samples}  &{\bf Description}  &{\bf \algName}  &{\bf SL }  &{\bf CEM}  &{\bf QL} \\
 & & &{\bf $\greedyEuc$}  &{\bf $\greedyMan$}  &{\bf WA*}  &{\bf MHA*} \\ \hline 
 
{switching doors} &
\multirow{2}{*}{\raisebox{-0.5\totalheight}{\setlength{\fboxsep}{0pt}
		\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/alternating_gaps/1.png}}} 
	\raisebox{-0.5\totalheight}{\setlength{\fboxsep}{0pt}
		\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/alternating_gaps/2.png}}} 
	\raisebox{-0.5\totalheight}{\setlength{\fboxsep}{0pt}
		\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/alternating_gaps/3.png}}}}
  & &$385.69$ & $2272.92$ & $403.44$ &  \\  
  & & &$0$ & $0$ & $0$ & $0$ \\ \hline 

{single bugtrap} &
\multirow{2}{*}{\raisebox{-0.5\totalheight}{\setlength{\fboxsep}{0pt}
		\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/bugtrap_world/1.png}}} 
	\raisebox{-0.5\totalheight}{\setlength{\fboxsep}{0pt}
		\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/bugtrap_world/2.png}}} 
	\raisebox{-0.5\totalheight}{\setlength{\fboxsep}{0pt}
		\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/bugtrap_world/3.png}}}}
& & & $1225.69$ &  &  \\  
& & &$0$ & $0$ & $0$ & $0$ \\ \hline 

{shifting door} &
\multirow{2}{*}{\raisebox{-0.5\totalheight}{\setlength{\fboxsep}{0pt}
		\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/shifting_gap/1.png}}} 
	\raisebox{-0.5\totalheight}{\setlength{\fboxsep}{0pt}
		\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/shifting_gap/2.png}}} 
	\raisebox{-0.5\totalheight}{\setlength{\fboxsep}{0pt}
		\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/shifting_gap/3.png}}}}
& &$699.92$ & $2426.98$ & $20000$ & $20000$ \\  
& & &$0$ & $0$ & $0$ & $0$ \\ \hline 

{forest} &
\multirow{2}{*}{\raisebox{-0.5\totalheight}{\setlength{\fboxsep}{0pt}
		\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/forest_world/1.png}}} 
	\raisebox{-0.5\totalheight}{\setlength{\fboxsep}{0pt}
		\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/forest_world/2.png}}} 
	\raisebox{-0.5\totalheight}{\setlength{\fboxsep}{0pt}
		\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/forest_world/3.png}}}}
& &$373.08$ & $406.029$ & $429.45$ &  \\  
& & &$0$ & $0$ & $0$ & $0$ \\ \hline 

{bugtrap+forest} &
\multirow{2}{*}{\raisebox{-0.5\totalheight}{\setlength{\fboxsep}{0pt}
		\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/bugtrap_forest/1.png}}} 
	\raisebox{-0.5\totalheight}{\setlength{\fboxsep}{0pt}
		\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/bugtrap_forest/2.png}}} 
	\raisebox{-0.5\totalheight}{\setlength{\fboxsep}{0pt}
		\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/bugtrap_forest/3.png}}}}
& &$903.78$ & $2045.43$ & $1069.75$ &  \\  
& & &$0$ & $0$ & $0$ & $0$ \\ \hline

{gaps+forest} &
\multirow{2}{*}{\raisebox{-0.5\totalheight}{\setlength{\fboxsep}{0pt}
		\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/gap_world/1.png}}} 
	\raisebox{-0.5\totalheight}{\setlength{\fboxsep}{0pt}
		\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/gap_world/2.png}}} 
	\raisebox{-0.5\totalheight}{\setlength{\fboxsep}{0pt}
		\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/gap_world/3.png}}}}
& &$1261.16$ & $8825.53$ & $15738.62$ &  \\  
& & &$0$ & $0$ & $0$ & $0$ \\ \hline 

{maze world} &
\multirow{2}{*}{\raisebox{-0.5\totalheight}{\setlength{\fboxsep}{0pt}
		\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/maze_world/1.png}}} 
	\raisebox{-0.5\totalheight}{\setlength{\fboxsep}{0pt}
		\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/maze_world/2.png}}} 
	\raisebox{-0.5\totalheight}{\setlength{\fboxsep}{0pt}
		\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/maze_world/3.png}}}}
& &$695.15$ & $1484.97$ & $2499.63$ &$2117.38$  \\  
& & &$0$ & $0$ & $0$ & $0$ \\ \hline 

{multiple bugtraps} &
\multirow{2}{*}{\raisebox{-0.5\totalheight}{\setlength{\fboxsep}{0pt}
		\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/multiple_bugtrap_world/1.png}}} 
	\raisebox{-0.5\totalheight}{\setlength{\fboxsep}{0pt}
		\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/multiple_bugtrap_world/2.png}}} 
	\raisebox{-0.5\totalheight}{\setlength{\fboxsep}{0pt}
		\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/multiple_bugtrap_world/3.png}}}}
& &$2501.34$ & $2503.42$ & $8145.94$ & $4209.23$ \\  
& & &$0$ & $0$ & $0$ & $0$ \\  
\bottomrule
\end{tabulary}
\label{tab:benchmark_results}
\end{table*}
 
% {bugtrap world} &
% \raisebox{-\totalheight}{\setlength{\fboxsep}{0pt}
% 	\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/bugtrap_world/1.png}}} 
% \raisebox{-\totalheight}{\setlength{\fboxsep}{0pt}
% 	\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=4mm]{figures/database_samples/bugtrap_world/2.png}}} 
% \raisebox{-\totalheight}{\setlength{\fboxsep}{0pt}
% 	\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/bugtrap_world/3.png}}} 
% &&&&&\\ \hline
%% &&&&&\\ \hline
% 
%  {shifting door} &
%  \raisebox{-\totalheight}{\setlength{\fboxsep}{0pt}
%  	\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/shifting_gap/1.png}}} 
%  \raisebox{-\totalheight}{\setlength{\fboxsep}{0pt}
%  	\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/shifting_gap/2.png}}} 
%  \raisebox{-\totalheight}{\setlength{\fboxsep}{0pt}
%  	\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/shifting_gap/3.png}}}
%  &&&&&\\ \hline
%%  &&&&&\\ \hline
% {forest world}&
% \raisebox{-\totalheight}{\setlength{\fboxsep}{0pt}
% 	\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/forest_world/1.png}}} 
% \raisebox{-\totalheight}{\setlength{\fboxsep}{0pt}
% 	\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/forest_world/2.png}}} 
% \raisebox{-\totalheight}{\setlength{\fboxsep}{0pt}
% 	\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/forest_world/3.png}}} 
% &&&&& \\ \hline
%% &&&&&\\ \hline
% {gap world}&
% \raisebox{-\totalheight}{\setlength{\fboxsep}{0pt}
% 	\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/gap_world/1.png}}} 
% \raisebox{-\totalheight}{\setlength{\fboxsep}{0pt}
% 	\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/gap_world/2.png}}} 
% \raisebox{-\totalheight}{\setlength{\fboxsep}{0pt}
% 	\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/gap_world/3.png}}}
% &&&&& \\ \hline
%% &&&&&\\ \hline
% {bugtrap forest}&
%  \raisebox{-\totalheight}{\setlength{\fboxsep}{0pt}
% 	\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/bugtrap_forest/1.png}}} 
% \raisebox{-\totalheight}{\setlength{\fboxsep}{0pt}
% 	\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/bugtrap_forest/2.png}}} 
% \raisebox{-\totalheight}{\setlength{\fboxsep}{0pt}
% 	\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/bugtrap_forest/3.png}}}
% &&&&& \\ \hline
%% &&&&&\\ \hline
% {maze world}&
%   \raisebox{-\totalheight}{\setlength{\fboxsep}{0pt}
% 	\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/maze_world/1.png}}} 
% \raisebox{-\totalheight}{\setlength{\fboxsep}{0pt}
% 	\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/maze_world/2.png}}} 
% \raisebox{-\totalheight}{\setlength{\fboxsep}{0pt}
% 	\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/maze_world/3.png}}}
% &&&&& \\ \hline
%% &&&&&\\ \hline
% {multiple bugtraps}&
%   \raisebox{-\totalheight}{\setlength{\fboxsep}{0pt}
% 	\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/multiple_bugtrap_world/1.png}}} 
% \raisebox{-\totalheight}{\setlength{\fboxsep}{0pt}
% 	\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/multiple_bugtrap_world/2.png}}} 
% \raisebox{-\totalheight}{\setlength{\fboxsep}{0pt}
% 	\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/multiple_bugtrap_world/3.png}}}
% &&&&& \\
% &&&&&\\

%\begin{tabulary}{\textwidth}{LCCCCCCCCCCC}\toprule
%       & {\bf \algMVOI}       & {\bf \algRandom}       & {\bf \algMaxTally}       & {\bf \algSetCover}    & {\bf \algName} \\ 
%       &                      & {Unconstrained}    & {Unconstrained}   & {Unconstrained}   & {Unconstrained}               \\
%       &                      & {MaxProbReg}        & {MaxProbReg}      & {MaxProbReg}      & {MaxProbReg}                 \\ \midrule
%\multicolumn{6}{c}{ {\bf Synthetic Bernoulli Test: Variation across region overlap} }   \\
%Small
%            &                   & $(4.18, 6.67)$  & $(3.49, 5.23)$  & $(1.77, 3.01)$  & $(1.42, 2.36)$    \\
%$\numRegion:100$
%            & $(0.00, 0.08)$     & $(0.12, 0.29)$  & $(0.12, 0.25)$  & $(0.18, 0.40)$  & $\red(0.00, 0.00)$  \\ 
%Medium
%            &                   & $(3.27, 4.40)$  & $(3.04, 4.30)$  & $(3.55, 4.67)$  & $(1.77, 2.64)$   \\
%$\numRegion:500$  
%            & $\red(0.00, 0.00)$& $(0.05, 0.25)$  & $(0.14, 0.24)$  & $(0.14, 0.33)$  & $\red(0.00, 0.00)$  \\ 
%Large
%            &                   & $(2.86, 4.26)$  & $(2.62, 3.85)$  & $(2.94, 3.71)$  & $(1.33, 1.81)$   \\
%$\numRegion:1000$
%            & $\red(-0.11, 0.00)$& $(0.00, 0.28)$ & $(0.06, 0.26)$  & $(0.09, 0.22)$  & $(0.00, 0.00)$   \\
%\multicolumn{6}{c}{ {\bf 2D Geometric Planning: Variation across environments} }   \\
%Forest    &                   & $(19.45, 27.66)$  & $(4.68, 6.55)$  & $(3.53, 5.07)$   & $(1.90, 2.46)$    \\
%          & $(0.03, 0.18)$    & $(0.13, 0.30)$    & $(0.09, 0.18)$  & $(0.00, 0.09)$   & $\red(0.00, 0.00)$   \\ 
%OneWall   &                   & $(13.35, 17.79)$  & $(4.12, 4.89)$   & $(1.36, 2.11)$    & $(0.76, 1.20)$    \\ 
%          & $(0.045, 0.21)$   & $(0.11, 0.42)$    & $(0.00, 0.12)$   & $(0.14, 0.29)$    & $\red(0.00, 0.00)$  \\ 
%TwoWall   &                   & $(13.76, 16.61)$  & $(2.76, 3.93)$   & $(2.07, 2.94)$    & $(0.91, 1.44)$    \\
%          & $(0.00, 0.09)$    & $(0.33, 0.51)$    & $(0.10, 0.20)$   & $\red(0.00, 0.00)$    & $\red(0.00, 0.00)$\\
%\multicolumn{6}{c}{ {\bf 2D Geometric Planning: Variation across region size} }   \\
%OneWall    &                  & $(12.06, 16.01)$  & $(4.47, 5.13)$  & $(2.00, 3.41)$   & $(0.94, 1.42)$    \\
%$\numRegion:300$
%          & $(0.00, 0.17)$    & $(0.12, 0.42)$    & $(0.06, 0.24)$  & $(0.00, 0.38)$   & $\red(0.00, 0.00)$  \\ 
%OneWall   &                   & $(13.26, 16.79)$  & $(2.18, 3.77)$   & $(1.04, 1.62)$    & $(0.41, 0.91)$    \\ 
%$\numRegion:858$ 
%          & $(0.00, 0.14)$   & $(0.09, 0.27)$    & $\red(-0.04, 0.08)$   & $(0.00, 0.14)$    & $\red(0.00, 0.00)$  \\ 
%\multicolumn{6}{c}{ {\bf Non-holonomic Path Planning: Variation across environments} }   \\
%Forest    &                   & $(22.38, 29.67)$  & $(9.79, 11.14)$    & $(2.63, 5.28)$ & $(1.54, 2.46)$  \\
%          & $(0.09, 0.18 )$   & $(0.46, 0.79)$    & $(0.25, 0.38)$     & $\red(0.00, 0.00)$ & $\red(0.00, 0.00)$\\ 
%OneWall   &                   & $(13.02, 15.75)$  & $(8.40, 11.47)$    & $(3.72, 4.54)$   & $(3.28, 3.78)$    \\ 
%          & $\red(-0.11, 0.11)$& $(0.00, 0.12)$    & $(0.21, 0.28)$    & $\red(-0.11, 0.11)$  & $\red(0.00, 0.00) $ \\ 
%\multicolumn{6}{c}{ {\bf Non-holonomic Path Planning: Variation across lattice degree} }   \\
%OneWall    &                    & $(10.46, 11.57)$  & $(3.95, 4.83)$  & $(0.83, 1.18)$   & $(0.24, 0.58)$    \\
%$\degree:12$ & $(0.04, 0.11)$   & $(0.30, 0.56)$    & $(0.11, 0.18)$  & $(0.00, 0.06)$   & $\red(0.00, 0.00)$  \\ 
%OneWall    &                    & $(14.97, 17.90)$  & $(9.19, 13.11)$ & $(3.22, 5.07)$   & $(2.16, 2.81)$    \\
%$\degree:30$ & $(0.05, 0.10)$   & $(0.14, 0.40)$    & $(0.20, 0.52)$  & $(0.00, 0.03)$   & $\red(0.00, 0.00)$\\ 
%\multicolumn{6}{c}{ {\bf 7D Arm Planning: Variation across environments} }   \\ 
%Table     &                   & $(15.12, 19.41)$  & $(4.80, 6.98)$      & $(1.36, 2.17)$      & $(0.32, 0.67)$    \\ 
%          & $(0.28, 0.54)$    & $(0.13, 0.31)$    & $(0.00, 0.04)$      & $(0.00, 0.11)$      & $\red(0.00, 0.00)$  \\ 
%Clutter   &                   & $(7.92, 9.85)$    & $(3.96, 6.44)$      & $(1.42, 2.07)$      & $(1.23, 1.75)$    \\
%          &$(0.02, 0.20)$     & $(0.14, 0.36)$    & $\red(0.00, 0.00)$  & $(0.00, 0.11)$      & $\red(0.00, 0.00)$ \\ \bottomrule
%\end{tabulary}


==> figures/table_32dim_eval.tex <==
\begin{table*}[!htpb]
\small
\centering
\caption{Sum of expansions over test set on different datasets- 32x32 images}
\begin{tabulary}{1.0\textwidth}{LC|*{5}{C}} \toprule
 & {\bf World Samples} &{\bf Pruning}  &{\bf Pruning }  &{\bf Recursive}  &{\bf A*} &{\bf Optimal}\\
 & &{\bf $\tau=0.5$}  &{\bf $\tau_{opt}$}  &{\bf }  &{\bf $\greedyEuc$} &{\bf }\\ \hline 
 
{alternating gaps} &
\multirow{2}{*}{\raisebox{-0.5\totalheight}{\setlength{\fboxsep}{0pt}
		\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/alternating_gaps/1.png}}} 
	\raisebox{-0.5\totalheight}{\setlength{\fboxsep}{0pt}
		\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/alternating_gaps/2.png}}} 
	\raisebox{-0.5\totalheight}{\setlength{\fboxsep}{0pt}
		\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/alternating_gaps/3.png}}}}
 &$4939$ & $4152$ & $4152$ &  $11863$ & $4141$ \\
  &$ $ & $ $ & $ $ &  $ $ & $ $\\ \hline

{shifting gaps} &
\multirow{2}{*}{\raisebox{-0.5\totalheight}{\setlength{\fboxsep}{0pt}
		\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/shifting_gap/1.png}}} 
	\raisebox{-0.5\totalheight}{\setlength{\fboxsep}{0pt}
		\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/shifting_gap/2.png}}} 
	\raisebox{-0.5\totalheight}{\setlength{\fboxsep}{0pt}
		\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/shifting_gap/3.png}}}}
 &$/$ & $3884$ & $3884$ &  $9705$ & $3884$ \\
  &$ $ & $ $ & $ $ &  $ $ & $ $\\ \hline


{single bugtrap} &
\multirow{2}{*}{\raisebox{-0.5\totalheight}{\setlength{\fboxsep}{0pt}
		\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/bugtrap_world/1.png}}} 
	\raisebox{-0.5\totalheight}{\setlength{\fboxsep}{0pt}
		\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/bugtrap_world/2.png}}} 
	\raisebox{-0.5\totalheight}{\setlength{\fboxsep}{0pt}
		\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/bugtrap_world/3.png}}}}
 &$4433$ & $4161$ & $4007$ &  $6046$ & $3856$\\
  &$ $ & $ $ & $ $ &  $ $ & $ $\\ \hline

{shifting gaps} &
\multirow{2}{*}{\raisebox{-0.5\totalheight}{\setlength{\fboxsep}{0pt}
		\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/shifting_gap/1.png}}} 
	\raisebox{-0.5\totalheight}{\setlength{\fboxsep}{0pt}
		\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/shifting_gap/2.png}}} 
	\raisebox{-0.5\totalheight}{\setlength{\fboxsep}{0pt}
		\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/shifting_gap/3.png}}}}
 &$4177$ & $3909$ & $3909$ &  $11813$ & $3884$ \\
  &$ $ & $ $ & $ $ &  $ $ & $ $\\ \hline
{forest} &
\multirow{2}{*}{\raisebox{-0.5\totalheight}{\setlength{\fboxsep}{0pt}
		\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/forest_world/1.png}}} 
	\raisebox{-0.5\totalheight}{\setlength{\fboxsep}{0pt}
		\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/forest_world/2.png}}} 
	\raisebox{-0.5\totalheight}{\setlength{\fboxsep}{0pt}
		\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/forest_world/3.png}}}}
 &$3889$ & $3810$ & $3852$ &  $3686$ & $3493$ \\
  &$ $ & $ $ & $ $ &  $ $ & $ $\\ \hline
{bugtrap+forest} &
\multirow{2}{*}{\raisebox{-0.5\totalheight}{\setlength{\fboxsep}{0pt}
		\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/bugtrap_forest/1.png}}} 
	\raisebox{-0.5\totalheight}{\setlength{\fboxsep}{0pt}
		\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/bugtrap_forest/2.png}}} 
	\raisebox{-0.5\totalheight}{\setlength{\fboxsep}{0pt}
		\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/bugtrap_forest/3.png}}}}
 &$5785$ & $5551$ & $4487$ &  $7650$ & $3936$ \\
  &$ $ & $ $ & $ $ &  $ $ & $ $\\ \hline
{gaps+forest} &
\multirow{2}{*}{\raisebox{-0.5\totalheight}{\setlength{\fboxsep}{0pt}
		\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/gap_world/1.png}}} 
	\raisebox{-0.5\totalheight}{\setlength{\fboxsep}{0pt}
		\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/gap_world/2.png}}} 
	\raisebox{-0.5\totalheight}{\setlength{\fboxsep}{0pt}
		\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/gap_world/3.png}}}}
 &$18846$ & $18381$ & $14542$ &  $25688$ & $7111$ \\
  &$ $ & $ $ & $ $ &  $ $ & $ $\\ \hline
{maze world} &
\multirow{2}{*}{\raisebox{-0.5\totalheight}{\setlength{\fboxsep}{0pt}
		\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/maze_world/1.png}}} 
	\raisebox{-0.5\totalheight}{\setlength{\fboxsep}{0pt}
		\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/maze_world/2.png}}} 
	\raisebox{-0.5\totalheight}{\setlength{\fboxsep}{0pt}
		\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/maze_world/3.png}}}}
 &$5468$ & $5308$ & $4951$ &  $5988$ & $4147$ \\
  &$ $ & $ $ & $ $ &  $ $ & $ $\\ \hline

{multiple bugtraps} &
\multirow{2}{*}{\raisebox{-0.5\totalheight}{\setlength{\fboxsep}{0pt}
		\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/multiple_bugtrap_world/1.png}}} 
	\raisebox{-0.5\totalheight}{\setlength{\fboxsep}{0pt}
		\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/multiple_bugtrap_world/2.png}}} 
	\raisebox{-0.5\totalheight}{\setlength{\fboxsep}{0pt}
		\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/multiple_bugtrap_world/3.png}}}}
 &$6458$ & $6029$ & $5297$ &  $13302$ & $4351$ \\
  &$ $ & $ $ & $ $ &  $ $ & $ $\\ \hline
\bottomrule
\end{tabulary}
\label{tab:dim32_eval}
\end{table*}
 
% {bugtrap world} &
% \raisebox{-\totalheight}{\setlength{\fboxsep}{0pt}
% 	\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/bugtrap_world/1.png}}} 
% \raisebox{-\totalheight}{\setlength{\fboxsep}{0pt}
% 	\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=4mm]{figures/database_samples/bugtrap_world/2.png}}} 
% \raisebox{-\totalheight}{\setlength{\fboxsep}{0pt}
% 	\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/bugtrap_world/3.png}}} 
% &&&&&\\ \hline
%% &&&&&\\ \hline
% 
%  {shifting door} &
%  \raisebox{-\totalheight}{\setlength{\fboxsep}{0pt}
%  	\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/shifting_gap/1.png}}} 
%  \raisebox{-\totalheight}{\setlength{\fboxsep}{0pt}
%  	\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/shifting_gap/2.png}}} 
%  \raisebox{-\totalheight}{\setlength{\fboxsep}{0pt}
%  	\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/shifting_gap/3.png}}}
%  &&&&&\\ \hline
%%  &&&&&\\ \hline
% {forest world}&
% \raisebox{-\totalheight}{\setlength{\fboxsep}{0pt}
% 	\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/forest_world/1.png}}} 
% \raisebox{-\totalheight}{\setlength{\fboxsep}{0pt}
% 	\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/forest_world/2.png}}} 
% \raisebox{-\totalheight}{\setlength{\fboxsep}{0pt}
% 	\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/forest_world/3.png}}} 
% &&&&& \\ \hline
%% &&&&&\\ \hline
% {gap world}&
% \raisebox{-\totalheight}{\setlength{\fboxsep}{0pt}
% 	\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/gap_world/1.png}}} 
% \raisebox{-\totalheight}{\setlength{\fboxsep}{0pt}
% 	\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/gap_world/2.png}}} 
% \raisebox{-\totalheight}{\setlength{\fboxsep}{0pt}
% 	\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/gap_world/3.png}}}
% &&&&& \\ \hline
%% &&&&&\\ \hline
% {bugtrap forest}&
%  \raisebox{-\totalheight}{\setlength{\fboxsep}{0pt}
% 	\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/bugtrap_forest/1.png}}} 
% \raisebox{-\totalheight}{\setlength{\fboxsep}{0pt}
% 	\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/bugtrap_forest/2.png}}} 
% \raisebox{-\totalheight}{\setlength{\fboxsep}{0pt}
% 	\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/bugtrap_forest/3.png}}}
% &&&&& \\ \hline
%% &&&&&\\ \hline
% {maze world}&
%   \raisebox{-\totalheight}{\setlength{\fboxsep}{0pt}
% 	\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/maze_world/1.png}}} 
% \raisebox{-\totalheight}{\setlength{\fboxsep}{0pt}
% 	\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/maze_world/2.png}}} 
% \raisebox{-\totalheight}{\setlength{\fboxsep}{0pt}
% 	\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/maze_world/3.png}}}
% &&&&& \\ \hline
%% &&&&&\\ \hline
% {multiple bugtraps}&
%   \raisebox{-\totalheight}{\setlength{\fboxsep}{0pt}
% 	\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/multiple_bugtrap_world/1.png}}} 
% \raisebox{-\totalheight}{\setlength{\fboxsep}{0pt}
% 	\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/multiple_bugtrap_world/2.png}}} 
% \raisebox{-\totalheight}{\setlength{\fboxsep}{0pt}
% 	\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/multiple_bugtrap_world/3.png}}}
% &&&&& \\
% &&&&&\\

%\begin{tabulary}{\textwidth}{LCCCCCCCCCCC}\toprule
%       & {\bf \algMVOI}       & {\bf \algRandom}       & {\bf \algMaxTally}       & {\bf \algSetCover}    & {\bf \algName} \\ 
%       &                      & {Unconstrained}    & {Unconstrained}   & {Unconstrained}   & {Unconstrained}               \\
%       &                      & {MaxProbReg}        & {MaxProbReg}      & {MaxProbReg}      & {MaxProbReg}                 \\ \midrule
%\multicolumn{6}{c}{ {\bf Synthetic Bernoulli Test: Variation across region overlap} }   \\
%Small
%            &                   & $(4.18, 6.67)$  & $(3.49, 5.23)$  & $(1.77, 3.01)$  & $(1.42, 2.36)$    \\
%$\numRegion:100$
%            & $(0.00, 0.08)$     & $(0.12, 0.29)$  & $(0.12, 0.25)$  & $(0.18, 0.40)$  & $\red(0.00, 0.00)$  \\ 
%Medium
%            &                   & $(3.27, 4.40)$  & $(3.04, 4.30)$  & $(3.55, 4.67)$  & $(1.77, 2.64)$   \\
%$\numRegion:500$  
%            & $\red(0.00, 0.00)$& $(0.05, 0.25)$  & $(0.14, 0.24)$  & $(0.14, 0.33)$  & $\red(0.00, 0.00)$  \\ 
%Large
%            &                   & $(2.86, 4.26)$  & $(2.62, 3.85)$  & $(2.94, 3.71)$  & $(1.33, 1.81)$   \\
%$\numRegion:1000$
%            & $\red(-0.11, 0.00)$& $(0.00, 0.28)$ & $(0.06, 0.26)$  & $(0.09, 0.22)$  & $(0.00, 0.00)$   \\
%\multicolumn{6}{c}{ {\bf 2D Geometric Planning: Variation across environments} }   \\
%Forest    &                   & $(19.45, 27.66)$  & $(4.68, 6.55)$  & $(3.53, 5.07)$   & $(1.90, 2.46)$    \\
%          & $(0.03, 0.18)$    & $(0.13, 0.30)$    & $(0.09, 0.18)$  & $(0.00, 0.09)$   & $\red(0.00, 0.00)$   \\ 
%OneWall   &                   & $(13.35, 17.79)$  & $(4.12, 4.89)$   & $(1.36, 2.11)$    & $(0.76, 1.20)$    \\ 
%          & $(0.045, 0.21)$   & $(0.11, 0.42)$    & $(0.00, 0.12)$   & $(0.14, 0.29)$    & $\red(0.00, 0.00)$  \\ 
%TwoWall   &                   & $(13.76, 16.61)$  & $(2.76, 3.93)$   & $(2.07, 2.94)$    & $(0.91, 1.44)$    \\
%          & $(0.00, 0.09)$    & $(0.33, 0.51)$    & $(0.10, 0.20)$   & $\red(0.00, 0.00)$    & $\red(0.00, 0.00)$\\
%\multicolumn{6}{c}{ {\bf 2D Geometric Planning: Variation across region size} }   \\
%OneWall    &                  & $(12.06, 16.01)$  & $(4.47, 5.13)$  & $(2.00, 3.41)$   & $(0.94, 1.42)$    \\
%$\numRegion:300$
%          & $(0.00, 0.17)$    & $(0.12, 0.42)$    & $(0.06, 0.24)$  & $(0.00, 0.38)$   & $\red(0.00, 0.00)$  \\ 
%OneWall   &                   & $(13.26, 16.79)$  & $(2.18, 3.77)$   & $(1.04, 1.62)$    & $(0.41, 0.91)$    \\ 
%$\numRegion:858$ 
%          & $(0.00, 0.14)$   & $(0.09, 0.27)$    & $\red(-0.04, 0.08)$   & $(0.00, 0.14)$    & $\red(0.00, 0.00)$  \\ 
%\multicolumn{6}{c}{ {\bf Non-holonomic Path Planning: Variation across environments} }   \\
%Forest    &                   & $(22.38, 29.67)$  & $(9.79, 11.14)$    & $(2.63, 5.28)$ & $(1.54, 2.46)$  \\
%          & $(0.09, 0.18 )$   & $(0.46, 0.79)$    & $(0.25, 0.38)$     & $\red(0.00, 0.00)$ & $\red(0.00, 0.00)$\\ 
%OneWall   &                   & $(13.02, 15.75)$  & $(8.40, 11.47)$    & $(3.72, 4.54)$   & $(3.28, 3.78)$    \\ 
%          & $\red(-0.11, 0.11)$& $(0.00, 0.12)$    & $(0.21, 0.28)$    & $\red(-0.11, 0.11)$  & $\red(0.00, 0.00) $ \\ 
%\multicolumn{6}{c}{ {\bf Non-holonomic Path Planning: Variation across lattice degree} }   \\
%OneWall    &                    & $(10.46, 11.57)$  & $(3.95, 4.83)$  & $(0.83, 1.18)$   & $(0.24, 0.58)$    \\
%$\degree:12$ & $(0.04, 0.11)$   & $(0.30, 0.56)$    & $(0.11, 0.18)$  & $(0.00, 0.06)$   & $\red(0.00, 0.00)$  \\ 
%OneWall    &                    & $(14.97, 17.90)$  & $(9.19, 13.11)$ & $(3.22, 5.07)$   & $(2.16, 2.81)$    \\
%$\degree:30$ & $(0.05, 0.10)$   & $(0.14, 0.40)$    & $(0.20, 0.52)$  & $(0.00, 0.03)$   & $\red(0.00, 0.00)$\\ 
%\multicolumn{6}{c}{ {\bf 7D Arm Planning: Variation across environments} }   \\ 
%Table     &                   & $(15.12, 19.41)$  & $(4.80, 6.98)$      & $(1.36, 2.17)$      & $(0.32, 0.67)$    \\ 
%          & $(0.28, 0.54)$    & $(0.13, 0.31)$    & $(0.00, 0.04)$      & $(0.00, 0.11)$      & $\red(0.00, 0.00)$  \\ 
%Clutter   &                   & $(7.92, 9.85)$    & $(3.96, 6.44)$      & $(1.42, 2.07)$      & $(1.23, 1.75)$    \\
%          &$(0.02, 0.20)$     & $(0.14, 0.36)$    & $\red(0.00, 0.00)$  & $(0.00, 0.11)$      & $\red(0.00, 0.00)$ \\ \bottomrule
%\end{tabulary}


==> figures/table_compare_normalized.tex <==
\begin{table*}[!htpb]
\small
\centering
\caption{Comparison of expanded nodes and open list sizes between pruning methods and cost-to-go methods. The metric for expanded nodes is the relative error in percentages between the number of expanded nodes and the optimal minimal number of expansions. The size of the open list is normalized by the theoretical maximum value (it being the whole map space- 32*32).}
\begin{tabulary}{1.0\textwidth}{LC|*{5}{C}} \toprule
 & {\bf World Samples} &{\bf $h_{ML}$} &{\bf Pruning} &{\bf Pruning+$h_{ML}$} &{\bf Recursive } &{\bf Recursive+$h_{ML}$}\\ \hline 

{alternating gaps} &
\multirow{2}{*}{\raisebox{-0.5\totalheight}{\setlength{\fboxsep}{0pt}
		\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/alternating_gaps/1.png}}} 
	\raisebox{-0.5\totalheight}{\setlength{\fboxsep}{0pt}
		\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/alternating_gaps/2.png}}} 
	\raisebox{-0.5\totalheight}{\setlength{\fboxsep}{0pt}
		\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/alternating_gaps/3.png}}}}
 & $0.845$ & \textbf{0.265} & $0.458 \downarrow$ &  $0.265$ & $0.458 \downarrow$ \\
 & & $0.386$ & \textbf{0.072} & $0.193 \downarrow$ &  $0.072$ & $0.458 \downarrow$ \\
 
 & &$0.118$ & \textbf{0.058} & $0.086 \downarrow$ &  $0.058$ & $0.086 \downarrow$\\ \hline


{single bugtrap} &
\multirow{2}{*}{\raisebox{-0.5\totalheight}{\setlength{\fboxsep}{0pt}
		\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/bugtrap_world/1.png}}} 
	\raisebox{-0.5\totalheight}{\setlength{\fboxsep}{0pt}
		\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/bugtrap_world/2.png}}} 
	\raisebox{-0.5\totalheight}{\setlength{\fboxsep}{0pt}
		\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/bugtrap_world/3.png}}}}
 &$2.619$ &$7.909$ &\textbf{2.515} $\uparrow$ &$3.915$ &$17.479 \uparrow$\\
 & &$0.120$ &$0.083$ &$0.119 \downarrow$ &\textbf{0.070} &$0.087 \downarrow$\\ \hline


{forest} &
\multirow{2}{*}{\raisebox{-0.5\totalheight}{\setlength{\fboxsep}{0pt}
		\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/forest_world/1.png}}} 
	\raisebox{-0.5\totalheight}{\setlength{\fboxsep}{0pt}
		\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/forest_world/2.png}}} 
	\raisebox{-0.5\totalheight}{\setlength{\fboxsep}{0pt}
		\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/forest_world/3.png}}}}
 &$13.054$ & $11.336$ & $15.030 \uparrow$ &  \textbf{10.227} & $18.923 \downarrow$ \\
 & &$0.113$ & $0.101$ &$0.108 \downarrow$ &\textbf{0.092} & $0.092 \downarrow$\\ \hline

{bugtrap+forest} &
\multirow{2}{*}{\raisebox{-0.5\totalheight}{\setlength{\fboxsep}{0pt}
		\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/bugtrap_forest/1.png}}} 
	\raisebox{-0.5\totalheight}{\setlength{\fboxsep}{0pt}
		\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/bugtrap_forest/2.png}}} 
	\raisebox{-0.5\totalheight}{\setlength{\fboxsep}{0pt}
		\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/bugtrap_forest/3.png}}}}
 &$23.323$ & $40.980$ & $32.977 \uparrow$ &  \textbf{13.998} & $24.593 \uparrow$ \\
 & &$0.122$ & $0.105$ & $0.122 \downarrow$ &  \textbf{0.085} & $0.092 \downarrow$\\ \hline


{gaps+forest} &
\multirow{2}{*}{\raisebox{-0.5\totalheight}{\setlength{\fboxsep}{0pt}
		\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/gap_world/1.png}}} 
	\raisebox{-0.5\totalheight}{\setlength{\fboxsep}{0pt}
		\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/gap_world/2.png}}} 
	\raisebox{-0.5\totalheight}{\setlength{\fboxsep}{0pt}
		\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/gap_world/3.png}}}}
 &$26.733$ & $130.670$ & $40.992 \uparrow$ &  $80.410$ & \textbf{20.194} $\downarrow$ \\
 & &$0.183$ & $0.114$ & $0.180 \downarrow$ &  \textbf{0.078} & $0.145 \downarrow$\\ \hline
 

{maze world} &
\multirow{2}{*}{\raisebox{-0.5\totalheight}{\setlength{\fboxsep}{0pt}
		\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/maze_world/1.png}}} 
	\raisebox{-0.5\totalheight}{\setlength{\fboxsep}{0pt}
		\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/maze_world/2.png}}} 
	\raisebox{-0.5\totalheight}{\setlength{\fboxsep}{0pt}
		\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/maze_world/3.png}}}}
 &\textbf{1.615} & $22.739$ & \textbf{1.663} $\uparrow$ &  $16.783$ & $1.687 \uparrow$ \\
 & &$0.125$ & $0.099$ & $0.120 \downarrow$ &  \textbf{0.069} & $0.091 \downarrow$\\ \hline

{multiple bugtraps} &
\multirow{2}{*}{\raisebox{-0.5\totalheight}{\setlength{\fboxsep}{0pt}
		\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/multiple_bugtrap_world/1.png}}} 
	\raisebox{-0.5\totalheight}{\setlength{\fboxsep}{0pt}
		\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/multiple_bugtrap_world/2.png}}} 
	\raisebox{-0.5\totalheight}{\setlength{\fboxsep}{0pt}
		\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/multiple_bugtrap_world/3.png}}}}
 &$130.085$ & $37.554$ & $70.075 \downarrow$ &  \textbf{21.742} & $96.046 \downarrow$ \\
 & &$0.118$ & $0.102$ & $0.109 \downarrow$ &  \textbf{0.071} & $0.077 \downarrow$\\ \hline
 

\bottomrule
\end{tabulary}
\label{tab:normed_comp}
\end{table*}
 
% {bugtrap world} &
% \raisebox{-\totalheight}{\setlength{\fboxsep}{0pt}
% 	\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/bugtrap_world/1.png}}} 
% \raisebox{-\totalheight}{\setlength{\fboxsep}{0pt}
% 	\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=4mm]{figures/database_samples/bugtrap_world/2.png}}} 
% \raisebox{-\totalheight}{\setlength{\fboxsep}{0pt}
% 	\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/bugtrap_world/3.png}}} 
% &&&&&\\ \hline
%% &&&&&\\ \hline
% 
%  {shifting door} &
%  \raisebox{-\totalheight}{\setlength{\fboxsep}{0pt}
%  	\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/shifting_gap/1.png}}} 
%  \raisebox{-\totalheight}{\setlength{\fboxsep}{0pt}
%  	\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/shifting_gap/2.png}}} 
%  \raisebox{-\totalheight}{\setlength{\fboxsep}{0pt}
%  	\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/shifting_gap/3.png}}}
%  &&&&&\\ \hline
%%  &&&&&\\ \hline
% {forest world}&
% \raisebox{-\totalheight}{\setlength{\fboxsep}{0pt}
% 	\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/forest_world/1.png}}} 
% \raisebox{-\totalheight}{\setlength{\fboxsep}{0pt}
% 	\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/forest_world/2.png}}} 
% \raisebox{-\totalheight}{\setlength{\fboxsep}{0pt}
% 	\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/forest_world/3.png}}} 
% &&&&& \\ \hline
%% &&&&&\\ \hline
% {gap world}&
% \raisebox{-\totalheight}{\setlength{\fboxsep}{0pt}
% 	\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/gap_world/1.png}}} 
% \raisebox{-\totalheight}{\setlength{\fboxsep}{0pt}
% 	\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/gap_world/2.png}}} 
% \raisebox{-\totalheight}{\setlength{\fboxsep}{0pt}
% 	\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/gap_world/3.png}}}
% &&&&& \\ \hline
%% &&&&&\\ \hline
% {bugtrap forest}&
%  \raisebox{-\totalheight}{\setlength{\fboxsep}{0pt}
% 	\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/bugtrap_forest/1.png}}} 
% \raisebox{-\totalheight}{\setlength{\fboxsep}{0pt}
% 	\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/bugtrap_forest/2.png}}} 
% \raisebox{-\totalheight}{\setlength{\fboxsep}{0pt}
% 	\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/bugtrap_forest/3.png}}}
% &&&&& \\ \hline
%% &&&&&\\ \hline
% {maze world}&
%   \raisebox{-\totalheight}{\setlength{\fboxsep}{0pt}
% 	\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/maze_world/1.png}}} 
% \raisebox{-\totalheight}{\setlength{\fboxsep}{0pt}
% 	\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/maze_world/2.png}}} 
% \raisebox{-\totalheight}{\setlength{\fboxsep}{0pt}
% 	\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/maze_world/3.png}}}
% &&&&& \\ \hline
%% &&&&&\\ \hline
% {multiple bugtraps}&
%   \raisebox{-\totalheight}{\setlength{\fboxsep}{0pt}
% 	\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/multiple_bugtrap_world/1.png}}} 
% \raisebox{-\totalheight}{\setlength{\fboxsep}{0pt}
% 	\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/multiple_bugtrap_world/2.png}}} 
% \raisebox{-\totalheight}{\setlength{\fboxsep}{0pt}
% 	\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/multiple_bugtrap_world/3.png}}}
% &&&&& \\
% &&&&&\\

%\begin{tabulary}{\textwidth}{LCCCCCCCCCCC}\toprule
%       & {\bf \algMVOI}       & {\bf \algRandom}       & {\bf \algMaxTally}       & {\bf \algSetCover}    & {\bf \algName} \\ 
%       &                      & {Unconstrained}    & {Unconstrained}   & {Unconstrained}   & {Unconstrained}               \\
%       &                      & {MaxProbReg}        & {MaxProbReg}      & {MaxProbReg}      & {MaxProbReg}                 \\ \midrule
%\multicolumn{6}{c}{ {\bf Synthetic Bernoulli Test: Variation across region overlap} }   \\
%Small
%            &                   & $(4.18, 6.67)$  & $(3.49, 5.23)$  & $(1.77, 3.01)$  & $(1.42, 2.36)$    \\
%$\numRegion:100$
%            & $(0.00, 0.08)$     & $(0.12, 0.29)$  & $(0.12, 0.25)$  & $(0.18, 0.40)$  & $\red(0.00, 0.00)$  \\ 
%Medium
%            &                   & $(3.27, 4.40)$  & $(3.04, 4.30)$  & $(3.55, 4.67)$  & $(1.77, 2.64)$   \\
%$\numRegion:500$  
%            & $\red(0.00, 0.00)$& $(0.05, 0.25)$  & $(0.14, 0.24)$  & $(0.14, 0.33)$  & $\red(0.00, 0.00)$  \\ 
%Large
%            &                   & $(2.86, 4.26)$  & $(2.62, 3.85)$  & $(2.94, 3.71)$  & $(1.33, 1.81)$   \\
%$\numRegion:1000$
%            & $\red(-0.11, 0.00)$& $(0.00, 0.28)$ & $(0.06, 0.26)$  & $(0.09, 0.22)$  & $(0.00, 0.00)$   \\
%\multicolumn{6}{c}{ {\bf 2D Geometric Planning: Variation across environments} }   \\
%Forest    &                   & $(19.45, 27.66)$  & $(4.68, 6.55)$  & $(3.53, 5.07)$   & $(1.90, 2.46)$    \\
%          & $(0.03, 0.18)$    & $(0.13, 0.30)$    & $(0.09, 0.18)$  & $(0.00, 0.09)$   & $\red(0.00, 0.00)$   \\ 
%OneWall   &                   & $(13.35, 17.79)$  & $(4.12, 4.89)$   & $(1.36, 2.11)$    & $(0.76, 1.20)$    \\ 
%          & $(0.045, 0.21)$   & $(0.11, 0.42)$    & $(0.00, 0.12)$   & $(0.14, 0.29)$    & $\red(0.00, 0.00)$  \\ 
%TwoWall   &                   & $(13.76, 16.61)$  & $(2.76, 3.93)$   & $(2.07, 2.94)$    & $(0.91, 1.44)$    \\
%          & $(0.00, 0.09)$    & $(0.33, 0.51)$    & $(0.10, 0.20)$   & $\red(0.00, 0.00)$    & $\red(0.00, 0.00)$\\
%\multicolumn{6}{c}{ {\bf 2D Geometric Planning: Variation across region size} }   \\
%OneWall    &                  & $(12.06, 16.01)$  & $(4.47, 5.13)$  & $(2.00, 3.41)$   & $(0.94, 1.42)$    \\
%$\numRegion:300$
%          & $(0.00, 0.17)$    & $(0.12, 0.42)$    & $(0.06, 0.24)$  & $(0.00, 0.38)$   & $\red(0.00, 0.00)$  \\ 
%OneWall   &                   & $(13.26, 16.79)$  & $(2.18, 3.77)$   & $(1.04, 1.62)$    & $(0.41, 0.91)$    \\ 
%$\numRegion:858$ 
%          & $(0.00, 0.14)$   & $(0.09, 0.27)$    & $\red(-0.04, 0.08)$   & $(0.00, 0.14)$    & $\red(0.00, 0.00)$  \\ 
%\multicolumn{6}{c}{ {\bf Non-holonomic Path Planning: Variation across environments} }   \\
%Forest    &                   & $(22.38, 29.67)$  & $(9.79, 11.14)$    & $(2.63, 5.28)$ & $(1.54, 2.46)$  \\
%          & $(0.09, 0.18 )$   & $(0.46, 0.79)$    & $(0.25, 0.38)$     & $\red(0.00, 0.00)$ & $\red(0.00, 0.00)$\\ 
%OneWall   &                   & $(13.02, 15.75)$  & $(8.40, 11.47)$    & $(3.72, 4.54)$   & $(3.28, 3.78)$    \\ 
%          & $\red(-0.11, 0.11)$& $(0.00, 0.12)$    & $(0.21, 0.28)$    & $\red(-0.11, 0.11)$  & $\red(0.00, 0.00) $ \\ 
%\multicolumn{6}{c}{ {\bf Non-holonomic Path Planning: Variation across lattice degree} }   \\
%OneWall    &                    & $(10.46, 11.57)$  & $(3.95, 4.83)$  & $(0.83, 1.18)$   & $(0.24, 0.58)$    \\
%$\degree:12$ & $(0.04, 0.11)$   & $(0.30, 0.56)$    & $(0.11, 0.18)$  & $(0.00, 0.06)$   & $\red(0.00, 0.00)$  \\ 
%OneWall    &                    & $(14.97, 17.90)$  & $(9.19, 13.11)$ & $(3.22, 5.07)$   & $(2.16, 2.81)$    \\
%$\degree:30$ & $(0.05, 0.10)$   & $(0.14, 0.40)$    & $(0.20, 0.52)$  & $(0.00, 0.03)$   & $\red(0.00, 0.00)$\\ 
%\multicolumn{6}{c}{ {\bf 7D Arm Planning: Variation across environments} }   \\ 
%Table     &                   & $(15.12, 19.41)$  & $(4.80, 6.98)$      & $(1.36, 2.17)$      & $(0.32, 0.67)$    \\ 
%          & $(0.28, 0.54)$    & $(0.13, 0.31)$    & $(0.00, 0.04)$      & $(0.00, 0.11)$      & $\red(0.00, 0.00)$  \\ 
%Clutter   &                   & $(7.92, 9.85)$    & $(3.96, 6.44)$      & $(1.42, 2.07)$      & $(1.23, 1.75)$    \\
%          &$(0.02, 0.20)$     & $(0.14, 0.36)$    & $\red(0.00, 0.00)$  & $(0.00, 0.11)$      & $\red(0.00, 0.00)$ \\ \bottomrule
%\end{tabulary}


==> figures/table_ctg_compare.tex <==
\begin{table*}[!htpb]
\small
\centering
\caption{Comparison of number of expanded nodes (upper value), length of the reconstructed paths (middle value) and open list sizes (lower value) on 8 datasets and 5 methods.}
\begin{tabulary}{1.0\textwidth}{LC|*{6}{C}} \toprule
 & {\bf World Samples} &{\bf $h_{ML}$} &{$\lambda_{PRN}$} &{\bf $\lambda_{PRN}+h_{ML}$} &{\bf $\lambda_{REC}$ } &{\bf $\lambda_{REC}+h_{ML}$} &{\bf $\greedyEuc$}\\ \hline 

{alternating gaps} &
\multirow{2}{*}{\raisebox{-0.5\totalheight}{\setlength{\fboxsep}{0pt}
		\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/alternating_gaps/1.png}}} 
	\raisebox{-0.5\totalheight}{\setlength{\fboxsep}{0pt}
		\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/alternating_gaps/2.png}}} 
	\raisebox{-0.5\totalheight}{\setlength{\fboxsep}{0pt}
		\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/alternating_gaps/3.png}}}}
 &$4176$ & \textbf{4152} & $4160 \downarrow$ &  \textbf{4152} & $4160 \downarrow$ & $18226$\\
 
 & &$4157$ & \textbf{4144} & $4149 \downarrow$ &  \textbf{4144} & $4149 \downarrow$ & $4277$\\
 
 & &$12125$ & \textbf{5993} & $8856 \downarrow$ &  \textbf{5993} & $8856 \downarrow$ & $12539$\\ \hline

{shifting gaps} &
\multirow{2}{*}{\raisebox{-0.5\totalheight}{\setlength{\fboxsep}{0pt}
		\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/shifting_gap/1.png}}} 
	\raisebox{-0.5\totalheight}{\setlength{\fboxsep}{0pt}
		\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/shifting_gap/2.png}}} 
	\raisebox{-0.5\totalheight}{\setlength{\fboxsep}{0pt}
		\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/shifting_gap/3.png}}}}
 &$3898$ & \textbf{3884} & $3892 \downarrow$ &  \textbf{3884} & $3892 \downarrow$ & 9705\\
 
 & &$3894$ & \textbf{3884} & $3886 \downarrow$ &  \textbf{3884} & $3886 \downarrow$ & $3943$\\
 
 & &$12249$ & \textbf{5436} & $8017 \downarrow$ &  \textbf{5436} & $8017 \downarrow$ & $11297$\\ \hline

{single bugtrap} &
\multirow{2}{*}{\raisebox{-0.5\totalheight}{\setlength{\fboxsep}{0pt}
		\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/bugtrap_world/1.png}}} 
	\raisebox{-0.5\totalheight}{\setlength{\fboxsep}{0pt}
		\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/bugtrap_world/2.png}}} 
	\raisebox{-0.5\totalheight}{\setlength{\fboxsep}{0pt}
		\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/bugtrap_world/3.png}}}}
 &$3957$ &$4161$ &\textbf{3953} $\downarrow$ &$4007$ &$4530 \uparrow$ & $6038$\\
 
 &  &$3903$ &$3894$ &$3905 \downarrow$ &\textbf{3890} &$3969 \uparrow$ & $4010$\\
 
 & &$12366$ &$8549$ &$12279 \downarrow$ &\textbf{7235} &$8961 \downarrow$ & $11118$\\ \hline


{forest} &
\multirow{2}{*}{\raisebox{-0.5\totalheight}{\setlength{\fboxsep}{0pt}
		\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/forest_world/1.png}}} 
	\raisebox{-0.5\totalheight}{\setlength{\fboxsep}{0pt}
		\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/forest_world/2.png}}} 
	\raisebox{-0.5\totalheight}{\setlength{\fboxsep}{0pt}
		\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/forest_world/3.png}}}}
 &$3949$ & $3889$ & $4018 \uparrow$ &  \textbf{3852} & $4154 \downarrow$ & $3682$\\
 
 & &$3705$ & \textbf{3559} & $3715 \uparrow$ &  $3581$ & $3752 \downarrow$ &$3595$\\
 
 & &$11669$ & $10365$ &$11355 \downarrow$ &\textbf{9486} & $10097 \downarrow$ &$10812$\\ \hline

{bugtrap+forest} &
\multirow{2}{*}{\raisebox{-0.5\totalheight}{\setlength{\fboxsep}{0pt}
		\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/bugtrap_forest/1.png}}} 
	\raisebox{-0.5\totalheight}{\setlength{\fboxsep}{0pt}
		\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/bugtrap_forest/2.png}}} 
	\raisebox{-0.5\totalheight}{\setlength{\fboxsep}{0pt}
		\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/bugtrap_forest/3.png}}}}
 &$4854$ & $5551$ & $5234 \uparrow$ &  \textbf{4487} & $4904 \uparrow$ &$7650$\\
 
 & &$4301$ & $4090$ & $4304 \uparrow$ &  \textbf{4025} & $4272 \uparrow$ &$4402$\\
 
 & &$12543$ & $10836$ & $12493 \downarrow$ &  \textbf{8730} & $9490 \downarrow$ &$10992$\\ \hline


{gaps+forest} &
\multirow{2}{*}{\raisebox{-0.5\totalheight}{\setlength{\fboxsep}{0pt}
		\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/gap_world/1.png}}} 
	\raisebox{-0.5\totalheight}{\setlength{\fboxsep}{0pt}
		\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/gap_world/2.png}}} 
	\raisebox{-0.5\totalheight}{\setlength{\fboxsep}{0pt}
		\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/gap_world/3.png}}}}
 &$9012$ & $18122$ & $10641 \uparrow$ &  $14298$ & \textbf{8698} $\downarrow$ &$25688$\\
 
 & &$7542$ & $7465$ & $7476 \uparrow$ &  \textbf{7325} & $7340 \downarrow$ &$8537$\\
 
 & &$18798$ & $11470$ & $18437 \downarrow$ &  \textbf{7839} & $14609 \downarrow$ &$11331$\\ \hline
 

{maze world} &
\multirow{2}{*}{\raisebox{-0.5\totalheight}{\setlength{\fboxsep}{0pt}
		\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/maze_world/1.png}}} 
	\raisebox{-0.5\totalheight}{\setlength{\fboxsep}{0pt}
		\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/maze_world/2.png}}} 
	\raisebox{-0.5\totalheight}{\setlength{\fboxsep}{0pt}
		\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/maze_world/3.png}}}}
 &\textbf{4214} & $5090$ & \textbf{4214} $\downarrow$ &  $4843$ & $4217 \uparrow$ &$5988$\\
 
 & &\textbf{4192} & $4259$ & $4193 \uparrow$ &  $4227$ & $4193 \uparrow$ &$4409$\\
 
 & &$12867$ & $10170$ & $12450 \downarrow$ &  \textbf{7126} & $9369 \downarrow$ &$10858$\\ \hline

{multiple bugtraps} &
\multirow{2}{*}{\raisebox{-0.5\totalheight}{\setlength{\fboxsep}{0pt}
		\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/multiple_bugtrap_world/1.png}}} 
	\raisebox{-0.5\totalheight}{\setlength{\fboxsep}{0pt}
		\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/multiple_bugtrap_world/2.png}}} 
	\raisebox{-0.5\totalheight}{\setlength{\fboxsep}{0pt}
		\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/multiple_bugtrap_world/3.png}}}}
 &$10011$ & $5985$ & $7400 \downarrow$ & \textbf{5297} & $8530 \downarrow$ &$13302$\\
 
 & &$4702$ & $4544$ & $4679 \downarrow$ &\textbf{4448} & $4534 \downarrow$ &$5069$\\
 
 & &$12179$ & $10322$ & $11236 \downarrow$ &  \textbf{7277} & $7940 \downarrow$ &$11374$\\ \hline
 

\bottomrule
\end{tabulary}
\label{tab:dim32_eval}
\end{table*}
 
% {bugtrap world} &
% \raisebox{-\totalheight}{\setlength{\fboxsep}{0pt}
% 	\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/bugtrap_world/1.png}}} 
% \raisebox{-\totalheight}{\setlength{\fboxsep}{0pt}
% 	\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=4mm]{figures/database_samples/bugtrap_world/2.png}}} 
% \raisebox{-\totalheight}{\setlength{\fboxsep}{0pt}
% 	\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/bugtrap_world/3.png}}} 
% &&&&&\\ \hline
%% &&&&&\\ \hline
% 
%  {shifting door} &
%  \raisebox{-\totalheight}{\setlength{\fboxsep}{0pt}
%  	\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/shifting_gap/1.png}}} 
%  \raisebox{-\totalheight}{\setlength{\fboxsep}{0pt}
%  	\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/shifting_gap/2.png}}} 
%  \raisebox{-\totalheight}{\setlength{\fboxsep}{0pt}
%  	\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/shifting_gap/3.png}}}
%  &&&&&\\ \hline
%%  &&&&&\\ \hline
% {forest world}&
% \raisebox{-\totalheight}{\setlength{\fboxsep}{0pt}
% 	\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/forest_world/1.png}}} 
% \raisebox{-\totalheight}{\setlength{\fboxsep}{0pt}
% 	\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/forest_world/2.png}}} 
% \raisebox{-\totalheight}{\setlength{\fboxsep}{0pt}
% 	\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/forest_world/3.png}}} 
% &&&&& \\ \hline
%% &&&&&\\ \hline
% {gap world}&
% \raisebox{-\totalheight}{\setlength{\fboxsep}{0pt}
% 	\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/gap_world/1.png}}} 
% \raisebox{-\totalheight}{\setlength{\fboxsep}{0pt}
% 	\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/gap_world/2.png}}} 
% \raisebox{-\totalheight}{\setlength{\fboxsep}{0pt}
% 	\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/gap_world/3.png}}}
% &&&&& \\ \hline
%% &&&&&\\ \hline
% {bugtrap forest}&
%  \raisebox{-\totalheight}{\setlength{\fboxsep}{0pt}
% 	\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/bugtrap_forest/1.png}}} 
% \raisebox{-\totalheight}{\setlength{\fboxsep}{0pt}
% 	\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/bugtrap_forest/2.png}}} 
% \raisebox{-\totalheight}{\setlength{\fboxsep}{0pt}
% 	\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/bugtrap_forest/3.png}}}
% &&&&& \\ \hline
%% &&&&&\\ \hline
% {maze world}&
%   \raisebox{-\totalheight}{\setlength{\fboxsep}{0pt}
% 	\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/maze_world/1.png}}} 
% \raisebox{-\totalheight}{\setlength{\fboxsep}{0pt}
% 	\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/maze_world/2.png}}} 
% \raisebox{-\totalheight}{\setlength{\fboxsep}{0pt}
% 	\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/maze_world/3.png}}}
% &&&&& \\ \hline
%% &&&&&\\ \hline
% {multiple bugtraps}&
%   \raisebox{-\totalheight}{\setlength{\fboxsep}{0pt}
% 	\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/multiple_bugtrap_world/1.png}}} 
% \raisebox{-\totalheight}{\setlength{\fboxsep}{0pt}
% 	\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/multiple_bugtrap_world/2.png}}} 
% \raisebox{-\totalheight}{\setlength{\fboxsep}{0pt}
% 	\setlength{\fboxrule}{1pt}\fbox{\includegraphics[width=0.04\textwidth, height=6mm]{figures/database_samples/multiple_bugtrap_world/3.png}}}
% &&&&& \\
% &&&&&\\

%\begin{tabulary}{\textwidth}{LCCCCCCCCCCC}\toprule
%       & {\bf \algMVOI}       & {\bf \algRandom}       & {\bf \algMaxTally}       & {\bf \algSetCover}    & {\bf \algName} \\ 
%       &                      & {Unconstrained}    & {Unconstrained}   & {Unconstrained}   & {Unconstrained}               \\
%       &                      & {MaxProbReg}        & {MaxProbReg}      & {MaxProbReg}      & {MaxProbReg}                 \\ \midrule
%\multicolumn{6}{c}{ {\bf Synthetic Bernoulli Test: Variation across region overlap} }   \\
%Small
%            &                   & $(4.18, 6.67)$  & $(3.49, 5.23)$  & $(1.77, 3.01)$  & $(1.42, 2.36)$    \\
%$\numRegion:100$
%            & $(0.00, 0.08)$     & $(0.12, 0.29)$  & $(0.12, 0.25)$  & $(0.18, 0.40)$  & $\red(0.00, 0.00)$  \\ 
%Medium
%            &                   & $(3.27, 4.40)$  & $(3.04, 4.30)$  & $(3.55, 4.67)$  & $(1.77, 2.64)$   \\
%$\numRegion:500$  
%            & $\red(0.00, 0.00)$& $(0.05, 0.25)$  & $(0.14, 0.24)$  & $(0.14, 0.33)$  & $\red(0.00, 0.00)$  \\ 
%Large
%            &                   & $(2.86, 4.26)$  & $(2.62, 3.85)$  & $(2.94, 3.71)$  & $(1.33, 1.81)$   \\
%$\numRegion:1000$
%            & $\red(-0.11, 0.00)$& $(0.00, 0.28)$ & $(0.06, 0.26)$  & $(0.09, 0.22)$  & $(0.00, 0.00)$   \\
%\multicolumn{6}{c}{ {\bf 2D Geometric Planning: Variation across environments} }   \\
%Forest    &                   & $(19.45, 27.66)$  & $(4.68, 6.55)$  & $(3.53, 5.07)$   & $(1.90, 2.46)$    \\
%          & $(0.03, 0.18)$    & $(0.13, 0.30)$    & $(0.09, 0.18)$  & $(0.00, 0.09)$   & $\red(0.00, 0.00)$   \\ 
%OneWall   &                   & $(13.35, 17.79)$  & $(4.12, 4.89)$   & $(1.36, 2.11)$    & $(0.76, 1.20)$    \\ 
%          & $(0.045, 0.21)$   & $(0.11, 0.42)$    & $(0.00, 0.12)$   & $(0.14, 0.29)$    & $\red(0.00, 0.00)$  \\ 
%TwoWall   &                   & $(13.76, 16.61)$  & $(2.76, 3.93)$   & $(2.07, 2.94)$    & $(0.91, 1.44)$    \\
%          & $(0.00, 0.09)$    & $(0.33, 0.51)$    & $(0.10, 0.20)$   & $\red(0.00, 0.00)$    & $\red(0.00, 0.00)$\\
%\multicolumn{6}{c}{ {\bf 2D Geometric Planning: Variation across region size} }   \\
%OneWall    &                  & $(12.06, 16.01)$  & $(4.47, 5.13)$  & $(2.00, 3.41)$   & $(0.94, 1.42)$    \\
%$\numRegion:300$
%          & $(0.00, 0.17)$    & $(0.12, 0.42)$    & $(0.06, 0.24)$  & $(0.00, 0.38)$   & $\red(0.00, 0.00)$  \\ 
%OneWall   &                   & $(13.26, 16.79)$  & $(2.18, 3.77)$   & $(1.04, 1.62)$    & $(0.41, 0.91)$    \\ 
%$\numRegion:858$ 
%          & $(0.00, 0.14)$   & $(0.09, 0.27)$    & $\red(-0.04, 0.08)$   & $(0.00, 0.14)$    & $\red(0.00, 0.00)$  \\ 
%\multicolumn{6}{c}{ {\bf Non-holonomic Path Planning: Variation across environments} }   \\
%Forest    &                   & $(22.38, 29.67)$  & $(9.79, 11.14)$    & $(2.63, 5.28)$ & $(1.54, 2.46)$  \\
%          & $(0.09, 0.18 )$   & $(0.46, 0.79)$    & $(0.25, 0.38)$     & $\red(0.00, 0.00)$ & $\red(0.00, 0.00)$\\ 
%OneWall   &                   & $(13.02, 15.75)$  & $(8.40, 11.47)$    & $(3.72, 4.54)$   & $(3.28, 3.78)$    \\ 
%          & $\red(-0.11, 0.11)$& $(0.00, 0.12)$    & $(0.21, 0.28)$    & $\red(-0.11, 0.11)$  & $\red(0.00, 0.00) $ \\ 
%\multicolumn{6}{c}{ {\bf Non-holonomic Path Planning: Variation across lattice degree} }   \\
%OneWall    &                    & $(10.46, 11.57)$  & $(3.95, 4.83)$  & $(0.83, 1.18)$   & $(0.24, 0.58)$    \\
%$\degree:12$ & $(0.04, 0.11)$   & $(0.30, 0.56)$    & $(0.11, 0.18)$  & $(0.00, 0.06)$   & $\red(0.00, 0.00)$  \\ 
%OneWall    &                    & $(14.97, 17.90)$  & $(9.19, 13.11)$ & $(3.22, 5.07)$   & $(2.16, 2.81)$    \\
%$\degree:30$ & $(0.05, 0.10)$   & $(0.14, 0.40)$    & $(0.20, 0.52)$  & $(0.00, 0.03)$   & $\red(0.00, 0.00)$\\ 
%\multicolumn{6}{c}{ {\bf 7D Arm Planning: Variation across environments} }   \\ 
%Table     &                   & $(15.12, 19.41)$  & $(4.80, 6.98)$      & $(1.36, 2.17)$      & $(0.32, 0.67)$    \\ 
%          & $(0.28, 0.54)$    & $(0.13, 0.31)$    & $(0.00, 0.04)$      & $(0.00, 0.11)$      & $\red(0.00, 0.00)$  \\ 
%Clutter   &                   & $(7.92, 9.85)$    & $(3.96, 6.44)$      & $(1.42, 2.07)$      & $(1.23, 1.75)$    \\
%          &$(0.02, 0.20)$     & $(0.14, 0.36)$    & $\red(0.00, 0.00)$  & $(0.00, 0.11)$      & $\red(0.00, 0.00)$ \\ \bottomrule
%\end{tabulary}


==> macros/packages.tex <==
%============================================================================
% The following packages can be found on http:\\www.ctan.org
% BIBTEX
%\usepackage{cite}
% BIBLATEX: \usepackage[style=IEEEtran,backend=bibtex]{biblatex}

\usepackage{graphicx}  % for pdf, bitmapped graphics files
\usepackage{array}
%\usepackage{epsfig}   % for postscript graphics files
%\usepackage{mathptmx} % assumes new font selection scheme installed
\usepackage{times}     % assumes new font selection scheme installed
\usepackage[fleqn]{amsmath}   % assumes amsmath package installed
\usepackage{amssymb}   % assumes amsmath package installed
%\usepackage{mathabx}   % for \widebar % Böse (font 3)
\usepackage{dsfont}
\usepackage{float}     % for placing with (H) at a specific position 
\usepackage{textgreek}
\usepackage[table]{xcolor}  % Färbige Tabellen
\usepackage{booktabs}       % Schöne Tabellen (dicke und dünne Linien)
\usepackage{filemod}        % für autoupdate bei geänderten tikz-grafiken
\usepackage{xifthen}
\usepackage[linesnumbered,ruled,vlined]{algorithm2e}
\usepackage{epstopdf}
\usepackage{subcaption}
\usepackage{paralist}
\usepackage{footnote}
%==============================================================================
% macro for executing a shell command immidiatly 
%\newcommand{\runmycommand}[1]{\immediate\write18{#1}}
% AUTOMATIC BIBTEX
\IfFileExists{\jobname.aux}% needs --enable-write18
             {\typeout{bibtex \jobname.aux}
              \immediate\write18{bibtex \jobname.aux}
              \typeout{*** AUTO RUNNING BIBTEX ***}}
             {\typeout{*********** Rerun for bibliography *************}}
%FOR BIBLATEX %\addbibresource{./IEEEabrv,./library}
             
% Pakete für Blockdiagramme und Diagramme
\usepackage{tikz}               % Achtung die Reihenfolge der Tikz Pakete ist
\usepackage{pgfplots}           % entscheidend!
\usepackage{pgfplotstable} 
\usepgfplotslibrary{groupplots}
\usepgfplotslibrary{units}
%\usetikzlibrary{spy}
\usetikzlibrary{shadows,positioning,arrows}
%\usetikzlibrary{shapes,shapes.multipart}
\usetikzlibrary{calc}
\usetikzlibrary{trees,fit,backgrounds}
%\usetikzlibrary{patterns,decorations.pathreplacing,decorations.pathmorphing}
%\usetikzlibrary{decorations.markings}
\usetikzlibrary{matrix}
\usetikzlibrary{shadows.blur,shapes.symbols}

%=================================================================================
\usepgfplotslibrary{external} % PDFs machen
\tikzexternalize[prefix=tikz_temp/]     % Unterordner für PDFs
\newcommand\autoupdateexternfigure[2]{  % MAKRO UM AUTOUPDATE ZU ERMÖGLICHEN
  \tikzsetnextfilename{#2}              % pdf-filename
  \filemodCmp{#1}{tikz_temp/#2.log}%    % prüft file datum 
  {\tikzset{external/force remake=true}}% erzwingt remake wenn log alt
  {}
}
%\tikzset{external/force remake} % immer alle Bilder neu machen
% Achtung für später: EPS-Grafiken können mit Tikz auch automatisch erstellt werden (siehe Internet)
% Tipps zu eps: auf http://tex.stackexchange.com/questions/8641/export-eps-figures-from-tikz
%=================================================================================

% Spezial Worttrennungen
\hyphenation{Last-rampen Betriebs-punkt}

%============================================================================
% PDF-Einstellungen
%\usepackage[ pdfauthor={Zlatan Ajanovic, Michael Stolz, Martin Horn}
%             ,pdftitle={A Novel Observer Concept for Embedded Drivetrain Applications}
%             ,pdfpagelayout=TwoPageLeft
%             ,pdfstartview  = {FitV}
%             %,pdfpagemode  = UseAttachments %OPEN ATTACHMENTS-VIEW IN PD
%             ,pdfpagelabels = true
%             ,linkcolor     = {black}
%             ,colorlinks    = {true} 
%             ,citecolor     = {black}
%             ,urlcolor      = {black}
%             ,bookmarks, bookmarksnumbered
%             %,bookmarksopen={true}, 
%             %,pagebackref  = true, backref = page     %% turn on backreferencing
%             ,plainpages    = false
%             ,hypertexnames = true
%             ]{hyperref}
%============================================================================
% Matrizen ------------------------------------------------------------------  
%\usepackage{arydshln}         % have dotted lines to separate matrix elements 
%\newcommand{\myhdots}{\hdashline[.4pt/1.5pt]}          % macro für punktierte

==> macros/symbols3.tex <==
\newcommand{\mymatrix}[1]{\mathbf{#1}}
\newcommand{\myvector}[1]{\mathbf{#1}}
\newcommand{\mytransf}[1]{#1}
\newcommand{\myfarg}[1]{\mbox{\footnotesize$({#1})$}}
\newcommand{\mysub}[1]{_{\!\:\!#1}}

\newcommand{\A}{\mymatrix{A}}
\newcommand{\B}{\mymatrix{B}}
\newcommand{\C}{\mymatrix{C}}
\newcommand{\D}{\mymatrix{D}}
\newcommand{\F}{\mymatrix{F}}
\newcommand{\E}{\mymatrix{E}}
\newcommand{\Mmass}{\mymatrix{M}}

\newcommand{\K}{\mymatrix{K}}
\newcommand{\Id}{\mymatrix{I}}
\newcommand{\G}{\mymatrix{G}}
\newcommand{\SM}{\mymatrix{S}}
\newcommand{\PHI}{\boldsymbol\Phi}
\newcommand{\XI}{\boldsymbol\Lambda}
\newcommand{\HH}{\mymatrix{H}}

\newcommand{\LL}{\mymatrix{L}}
\newcommand{\T}{\tau}
\newcommand{\TT}{\boldsymbol\tau}
\newcommand{\M}{\mymatrix{M}}
\newcommand{\R}{\mytransf{R}}
\newcommand{\PP}{\mymatrix{P}}
\newcommand{\x}{\myvector{x}}
\newcommand{\dd}{\myvector{d}}
\newcommand{\e}{\myvector{e}}
\newcommand{\f}{\myvector{f}}
\newcommand{\uu}{\myvector{u}}
\newcommand{\z}{\myvector{z}}
\newcommand{\rr}{\myvector{r}}  
\newcommand{\y}{\myvector{y}} 
\newcommand{\vv}{\myvector{v}} 
\newcommand{\V}{\mymatrix{V}}
\newcommand{\U}{\mytransf{U}}
\newcommand{\X}{\mymatrix{X}}
\newcommand{\Q}{\mytransf{Q}}
\newcommand{\Z}{\mytransf{Z}}
\newcommand{\w}{\myvector{w}}


\newcommand{\q}{\mathbf{q}}
\newcommand{\mylam}[2]{\lambda_{(\mathit{#1},#2)}}
\newcommand{\mytau}[2]{\tau_{(\mathit{#1},#2)}}

\newcommand{\Teng}{\T_{\!\mathit{eng}}}
\newcommand{\Tmot}{\T_{\!\mathit{eng}}}
\newcommand{\Tveh}{\T_{\!\mathit{veh}}}
\newcommand{\Tsft}{\T_{\!\mathit{sft}}}
\newcommand{\Tstck}{\T_{\mathit{l}}}
\newcommand{\TBstck}{{\boldsymbol\T}_{\!\mathit{l}}}

\newcommand{\seng}{\mathit{eng}}
\newcommand{\ssft}{\mathit{sft}}
\newcommand{\sgbx}{\mathit{gbx}}
\newcommand{\sveh}{\mathit{veh}}
\newcommand{\swhl}{\mathit{whl}}
\newcommand{\spri}{\mathit{pri}}
\newcommand{\ssec}{\mathit{sec}}
\newcommand{\skin}{\mathit{kin}}
\newcommand{\sstat}{\mathit{stat}}
\newcommand{\sstck}{\mathit{l}}
\newcommand{\sslip}{\mathit{s}}

\newcommand{\bigO}{\mathcal{O}}
\newcommand{\Dataset}{\mathcal{D}}

\newcommand{\OPEN}{\textsc{Open}}
%\newcommand{\OPEN}{\mathrm{O\!P\!E\!N}}
\newcommand{\CLOSED}{\textsc{Closed}}	
%\newcommand{\CLOSED}{\textit{C\!L\!O\!S\!E\!D}}	




==> macros/tikzStyles.tex <==
\tikzstyle{s} = [font = \footnotesize]

\tikzstyle{doppelpfeil} = [-latex,postaction={draw,shorten >=6pt,-latex}]
\tikzstyle{sarrowtip} = [>=latex]  
\tikzstyle{myarrowtip} = [>=implies] 

\tikzset{curveinscope/.style={every path/.style={draw=white, double distance=1pt, line width=2pt, double=black, text=black}}}

\DeclareRobustCommand{\myLine}[1]{
(\tikzset{external/export next=false}\begin{tikzpicture}%
\useasboundingbox (-0.2ex,0) rectangle (4.65ex,1ex);%
\draw[line width=0.3ex,#1](0,0.65ex)--(4.5ex,0.65ex);%
\end{tikzpicture})}



